An In-Memory Architecture for High-Performance Long-Read Pre-Alignment Filtering

With the recent move towards sequencing of accurate long reads, finding solutions that support efficient analysis of these reads becomes more necessary. The long execution time required for sequence alignment of long reads negatively affects genomic studies relying on sequence alignment. Although pre-alignment filtering as an extra step before alignment was recently introduced to mitigate sequence alignment for short reads, these filters do not work as efficiently for long reads. Moreover, even with efficient pre-alignment filters, the overall end-to-end (i.e., filtering + original alignment) execution time of alignment for long reads remains high, while the filtering step is now a major portion of the end-to-end execution time. Our paper makes three contributions. First, it identifies data movement of sequences between memory units and computing units as the main source of inefficiency for pre-alignment filters of long reads. This is because although filters reject many of these long sequencing pairs before they get to the alignment stage, they still require a huge cost regarding time and energy consumption for the large data transferred between memory and processor. Second, this paper introduces an adaptation of a short-read pre-alignment filtering algorithm suitable for long reads. We call this LongGeneGuardian. Finally, it presents Filter-Fuse as an architecture that supports LongGeneGuardian inside the memory. FilterFuse exploits the Computation-In-Memory computing paradigm, eliminating the cost of data movement in LongGeneGuardian. Our evaluations show that FilterFuse improves the execution time of filtering by 120.47x for long reads compared to State-of-the-Art (SoTA) filter, SneakySnake. FilterFuse also improves the end-to-end execution time of sequence alignment by up to 49.14x and 5207.63x compared to SneakySnake with SoTA aligner and only SoTA aligner, respectively.

==> Sections/12_algorithm_execution_on_hardware.tex <==
\subsubsection{Algorithm Execution on Accelerator}
\label{subsubsec:algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}

\filterfuselongreadacc executes \geneguardianlongreadalg as soon as loading the reference into the memory elements (the one-time load) and the read sequence into the query row of the mapping location found by seed generation is completed. \fig{\ref{fig:algorithm_flowchart_at_subarray-read_and_reference_mapping-sscim_algorithm_mapping_acchwsscim}} presents the process in which the final bit vector is generated entirely in the addressed sub-arrays


\begin{figure}[htbp]
\centering
    \includegraphics[width=1\linewidth]{Figures/algorithm_flowchart_at_subarray-read_and_reference_mapping-sscim_algorithm_mapping_acchwsscim.pdf}
    \caption{A flowchart demonstrating the algorithm process at the sub-array level.\dtodo{Font Size!}}
    \label{fig:algorithm_flowchart_at_subarray-read_and_reference_mapping-sscim_algorithm_mapping_acchwsscim}
\end{figure}

As an example, assume the input data presented in \tab{\ref{tab:example_pairing-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}}. This example uses the last 4 segments of example in \fig{\ref{fig:SSPart_True_Negative_TN_Example-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}}. In this example, we assume this pairing is part of a longer read.

\begin{table}[htbp]
\small
\scriptsize
\centering
% \renewcommand{\arraystretch}{1.2}

\begin{tabular}{|c|c|}
\hline
Read Sequence           & \texttt{TGTC TGAA ACTT ACGC}                                              \\ \hline
Reference Sequence      & \texttt{..GTTGACTCGAAACTTACACT..}                                                                                    \\ \hline
Correct Alignment       & \begin{tabular}[c]{@{}c@{}}\texttt{~~TG\textcolor{red}{T}C~TG\textcolor{green}{-}AA~ACTT~AC\textcolor{red}{G}C~~}\\   \texttt{~~|| |~|| ||~||||~|| |~}    \\ \texttt{GT~TG\textcolor{red}{A}C~TC\textcolor{green}{G}AA~ACTT~AC\textcolor{red}{A}C~T}\end{tabular} \\ \hline
Edit-distance           & 3                                                                                                             \\ \hline
Edit-distance Threshold & 2                                                                                                             \\ \hline
\end{tabular}
\caption{Example read-reference pairing.}
\label{tab:example_pairing-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}
\end{table}



\begin{figure}[htbp]
\centering
    \includegraphics[width=1\linewidth]{Figures/SSPart_True_Negative_TN_Example-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM.pdf}
    \caption{Example True Negative (TN) case in  \geneguardianlongreadalg.\dtodo{Font Size!}}
    \label{fig:SSPart_True_Negative_TN_Example-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}
\end{figure}


\textbf{Bitwise \gatexorop operation.} In this example, \filterfuselongreadacc assumes the read reference pairing is written entirely on a single sub-array tile group, with each segment of 4 base pairs (8 bits) written to a separate tile. The correct alignment of this pairing contains three edits. Two substitutions (colored red in \tab{\ref{tab:example_pairing-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}}) and a deletion (colored in green). We focus on the left-most segment (mapped to tile \#3), which contains a substitution error (`a' in the reference sequence is replaced by a `t'), and the third segment (mapped to tile \#1), which does not contain an edit. \fig{\ref{fig:example_tile_shift4_xor-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}} presents the \gatexorop-results of the second shift, which corresponds to `Ref <<1', as this iteration shows a mismatch in the first segment but a match in the third segment.

\begin{figure}[htbp]
\centering
    \includegraphics[width=1\linewidth]{Figures/example_tile_shift4_xor-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM.pdf}
    \caption{Example of the tile-level execution of the \gatexorop result between the read-segment and the <<1 shifted reference.\dtodo{Font Size!}}
    \label{fig:example_tile_shift4_xor-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}
\end{figure}



\filterfuselongreadacc combines the \gatexorop results of the tiles and passes them as input to the pairwise-\gateorop block. The output of this operation is put through the masking block, which, in our example, is not masked off any part of the pairing. This result is then used as the input of the \pdtcam. \fig{\ref{fig:example_tile_xor_or_mask-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}} demonstrates this process. % on the XOR results obtained for the example pairing. 



\begin{figure}[htbp]
\centering
    \includegraphics[width=1\linewidth]{Figures/example_tile_xor_or_mask-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM.pdf}
    \caption{Example of the pairwise-\gateorop operation and the masking process.\dtodo{Font Size!}}
    \label{fig:example_tile_xor_or_mask-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}
\end{figure}


\textbf{Pattern detection.} \filterfuselongreadacc uses \gatexorop results as an input to the series of \tcam{}s. In \geneguardianlongreadalg, one needs to find if any shifted Hamming mask of a segment contains only zeros, which indicates an exact match of that segment. The pattern that needs to be detected by the \pdtcam is, therefore, a series of zeros starting and ending at the beginning and end of each segment, respectively. The programming of the \pdtcam for a segment size of 4 \bp{}s is shown in \fig{\ref{fig:example_sspart_subarray_tcam-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}}. A `1' in the output of the \pdtcam indicates the existence of an exact match. For \filterfuselongreadacc, the final bit-vector should contain a `1' for every segment with no exact matches for any of its shifted Hamming distances. The \ostcam essentially creates this by inverting the intermediate result. In our example, all segments contain errors except for the third segment. The partial final bit-vector thus contains 3 `1's to indicate the presence of at least 3 edits.


\begin{figure}[htbp]
\centering
    \includegraphics[width=1\linewidth]{Figures/example_sspart_subarray_tcam-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM.pdf}
    \caption{Example programming of the \tcam{}s for \geneguardianlongreadalg with a segment size of 4 \bp{}s.\dtodo{Font Size!}}
    \label{fig:example_sspart_subarray_tcam-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}
\end{figure}


\textbf{Final bit-vector accumulation.} 

\filterfuselongreadacc collects the results of the \counttcam in a register and accumulates over all iterations of the reference shifts. It initializes this intermediate-result register to all `1's, which is used as an operand for the \gateandop-operation with the \ostcam output. The results of all iterations of the example pairing using \geneguardianlongreadalg are shown in \tab{\ref{tab:intermediate_SSCIM-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}}. Here, we use te gray color for the parts that do not contain useful information. After all the iterations are completed, the intermediate result is returned to the rank level for further processing, along with its corresponding ID.


\begin{table}[htbp]
\small
\scriptsize
\centering
% \renewcommand{\arraystretch}{1.2}

\begin{tabular}{|l|c|c|c|}
\hline
Iteration & Hamming mask       & \ostcam output    & Intermediate Result \\ \hline
0         & -                   & -                 & 1111 \textcolor{gray}{111111111111}   \\
1         & 1100 1100 1101 1111 & 1111 \textcolor{gray}{000000000000} & 1101 \textcolor{gray}{000000000000}   \\
2         & 1111 1000 0000 0010 & 1101 \textcolor{gray}{000000000000} & 1101 \textcolor{gray}{000000000000}   \\
3         & 1110 0110 0110 1111 & 1111 \textcolor{gray}{000000000000} & 1101 \textcolor{gray}{000000000000}   \\
4         & 0111 1111 0111 1110 & 1111 \textcolor{gray}{000000000000} & 1101 \textcolor{gray}{000000000000}   \\
5         & 1101 1111 1111 1111 & 1111 \textcolor{gray}{000000000000} & 1101 \textcolor{gray}{000000000000}   \\ \hline                            

\end{tabular}
\caption{The evolution of the intermediate result register over the iterations of \geneguardianlongreadalg (segment size 4).}
\label{tab:intermediate_SSCIM-algorithm_execution-sscim_algorithm_mapping_acchwsscim-proposed_architecture_hardware_accelerator_SSCIM}
\end{table}



\textbf{Edit counting.} \mscomment{Make the changes to the rank level to remove the tcam and include the adder instead.} \mscomment{You might also need a not series.}
At the rank level, \filterfuselongreadacc collects the results of all bank groups to count the number of edits in a word set of the read sequence. \filterfuselongreadacc does this using a multi-operand adder. \filterfuselongreadacc stores the resulting sum in integer representation in the sum buffer that is indexed by the ID. Once all word sets of the read sequence have been processed, \filterfuselongreadacc compares this total sum to the edit-distance threshold. The result of this comparison determines whether the pairing is passed or blocked. 

 


